Decision Approach and Empirical Bayes FCR-Controlling Interval for Mixed Prior Model

In this paper, I apply the decision theory and empirical Bayesian approach to construct confidence intervals for selected populations when true parameters follow a mixture prior distribution. A loss function with two tuning parameters $k_1$ and $k_2$ is coined to address the mixture prior. One specific choice of $k_2$ can lead to the procedure in Qiu and Hwang (2007); the other choice of $k_2$ provides an interval construction which controls the Bayes FCR. Both the analytical and extensive numerical simulation studies demonstrate that the new empirical Bayesian FCR controlling approach enjoys great length reduction. At the end, I apply different methods to a microarray data set. It turns out that the average length of the new approach is only 57% of that of Qiu and Hwang's procedure which controls the simultaneous non-coverage probability and 66% of that of Benjamini and Yekutieli (2005)'s procedure which controls the frequentist's FCR.

==> data.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "CIMixed"
%%% End:
In this section, I apply different intervals to a microarray data set, the Synteni data of Kerr, Martin, and Churchill (2000), which was
revisited by Hsu et al.(2006) and Qiu and Hwang (2007).
The description of the data set can be found in
Kerr, et al. (2000). The figure 6 of Qiu and Hwang (2007) is a Q-Q plot of the ANOVA estimator $X_g$, which shows that the
normal-mixture model (\ref{model:mixed}) fits the data well. 

Hsu et al. (2006) uses simultaneous confidence intervals to detect
genes with an expression level of $\Delta=3$ or more. I will
first apply Benjamini and Hochberg (1995)'s procedure to select
parameters with expression levels significantly larger or equal than
$\log_23$, and then construct the simultaneous interval for
such selected observations. B-H's procedure declares that the first 89 genes
are significant.

In figure \ref{fig:allinterval}, I construct the confidence intervals for these 89 genes
by using Qiu and Hwang (2007)'s, B-Y's, (\ref{interval:final:emBayes}).
Our confidence interval (\ref{interval:final:emBayes}) for $\theta_{(g)}$ is
$0.93X_{(g)}\pm 0.96$. Compared with the interval $X_{(g)}\pm
1.47$ of BY's procedure, $0.93X_{(g)}\pm 1.67$ of Qiu and Hwang
(2006), our intervals enjoy great length reduction.



==> discussion.tex <==
In this article, I have defined a new loss function for confidence
interval construction when assuming the mixed prior model (\ref{model:mixed}).
I use two different ways to choose the tuning parameter in the loss function
to obtain Qiu and Hwang (2007)'s procedure and the empirical Bayesian FCR controlling
intervals. I conclude that the new empirical Bayesian FCR controlling interval is
better than other existing procedures because of the sharp improvement over the average length.

However, there are still much need for further research. In model
(\ref{model:mixed}), I assume equal and known variance
$\sigma^2$, which is not generally a practical assumption. Hwang,
Qiu, and Zhao (2008) proposed a double shrinkage empirical
Bayesian interval for single
parameter without selection under the normal-lognormal model.
Therefore, one natural extension of this work is to consider the mixture-prior model
when variances are unequal and unknown. The loss function 
(\ref{model:loss}) provides us a potential tool to construct
corresponding intervals.


==> introduction.tex <==
Simultaneous interval estimation for a large number of selected
parameters is challenging especially when the number of
observations for each parameter is very small. The difficulties are
the selection bias (see Qiu and Hwang 2007 and Hwang 1993) and the
multiplicity. The traditional approach, which treats all the
parameters as fixed, seems to have little power when the dimension
tends to be very large, for instance, several thousands in
microarray. However, the empirical Bayesian approach is known to be able to
{\it borrow strength} across the populations. Thus, it is very
likely that this method will provide us with some satisfactory
procedures.

In the past, people attempted to estimate the parameters for selection
populations (see, for example, Cohen and Sackrowitz 1982
and Hwang 1993).
However, very few people knew how to construct an interval for
selected population. The first
exciting work was written by Benjamini and Yekutieli (2005) (I will use
B-Y (2005) to represent this work throughout the paper). They
adapted the concept of FDR from multiple testing and coined a
concept False Coverage Rate (FCR) for simultaneous intervals.
This criterion is much less conservative than the simultaneous non-coverage
coefficient. They have constructed confidence intervals for
multiple selected parameters which can control the FCR at
specified $q$-level, typically 5\%. They centered their intervals upon
the estimator $X_i$'s which are biased for selected populations and addressed the multiplicity
by lengthening the intervals. Consequently, their intervals have
extremely large average half length.

In 2008, Zhao and Hwang introduced the Bayes FCR and connected
Bayes confidence interval which aims at controlling Bayesian
non-coverage coefficients with the Bayesian FCR controlling intervals. They applied this
general theorem to the normal-normal setting where the observations
follow a normal distribution with unequal but know variances and the parameters
follow a normal prior. They used the
empirical Bayesian approach to derive explicit intervals which
can control the empirical Bayes FCR. 
Their construction reduced the average length of B-Y's procedure dramatically
because they addressed the multiplicity by modifying the centers instead of the lengths.

Another exciting work is Qiu and Hwang (2007), which offers a way
to construct intervals that can control
the simultaneous coverage coefficient for selected popultions.  Other than the
normal-normal model, they treated the so-called normal-mixture model
where the prior distribution of the true parameters is a mixture
of a normal random variable with an equal, known variance and a single point {\it zero}. Because
they have addressed the multiplicity by Bonferroni's correction,
their lengths tend to be large when many parameters are selected.

In this paper, I use the decision approach and empirical
Bayes to construct intervals for selected populations under the same model
setting of Qiu and Hwang (2007).
Application of decision approach to interval/set estimation has a
long history which dates back to Faith (1976), Casella and Hwang
(1983), and He (1992). Recently, Hwang, Qiu, and Zhao (2008) have
constructed the double shrinkage empirical confidence interval for
one single parameter when assuming the variances to be unequal and
unknown. However, all the loss functions they have used are not
appropriate under the mixed prior model (Detailed argument is in
section \ref{model:Bayes}). Thus a new loss function with two
tuning parameters $k_1$ and $k_2$ is proposed and strongly
recommended. One specific choice of $k_2$ results in Qiu and Hwang
(2007)'s procedure. The other choice of $k_2$ provides us with a
way to construct the empirical Bayesian FCR-controlling intervals
based on the normal-mixture model.

In section \ref{model}, I introduce the model setting and the
decision Bayes rule based on our new loss function. In section
\ref{FCR}, I will connect the decision Bayesian rule with Qiu and
Hwang (2007)'s procedure first and then derive a procedure which can control the Bayes
FCR. In section \ref{empirical}, empirical Bayesian approach is
constructed and evaluated both numerically and analytically. In
section \ref{data}, I apply the confidence intervals constructed in 
section \ref{empirical} to a real microarray
dataset and compare it with B-Y (2005)'s and Qiu and Hwang's procedures.
It turns out that my procedure out-performs theirs.
The average length of my
 interval is only 57\% of that of Qiu and Hwang's (2007) procedure which controls
the simultaneous coverage probability and 66\% 
of that of B-Y (2005)'s procedure which controls the frequentist's FCR.

